Improving estimates of the number of fake leptons and other mis-reconstructed objects in hadron collider events: BoB's your UNCLE. (Previously "The Matrix Method Reloaded")

We consider current and alternative approaches to setting limits on new physics signals having backgrounds from misidentified objects; for example jets misidentified as leptons, b-jets or photons. Many ATLAS and CMS analyses have used a heuristic matrix method for estimating the background contribution from such sources. We demonstrate that the matrix method suffers from statistical shortcomings that can adversely affect its ability to set robust limits. A rigorous alternative method is discussed, and is seen to produce fake rate estimates and limits with better qualities, but is found to be too costly to use. Having investigated the nature of the approximations used to derive the matrix method, we propose a third strategy that is seen to marry the speed of the matrix method to the performance and physicality of the more rigorous approach.

==> commands.tex <==
\RequirePackage{maybemath}
\RequirePackage{xspace}

\DeclareRobustCommand{\mymath}[1]{\ensuremath{\maybebmsf{#1}}}
\DeclareRobustCommand{\MathUpright}[1]{\mymath{\mathrm{#1}}}
\DeclareRobustCommand{\MathText}[1]{\ensuremath{\text{#1}}}


% Chris's acclaimed auto abbreviation awesomeness
 \def\mygloss#1#2#3{\glossary{#1 @{\bf #2} & #3}}
\newcommand{\prepareAbbrev}[6]{\newcounter{#5}\newcommand{#1}{\mygloss{#2}{#6}{#4}\ifnum\arabic{#5}=0 {#4 (#3)}\else#3\fi\addtocounter{#5}{1}}}
\prepareAbbrev\MLE{MLE}{MLE}{maximum likelihood estimate}{MLEcounter}{MLE}


% Editing convenience commands

\newcommand{\assum}[1]{\textbf{\color{red} Assumption[ {#1} ]}}
\newcommand{\comCGL}[1]{{\color{blue}[CGL: {#1}]}}
\newcommand{\comTPSG}[1]{{\color{green}[TPSG: {#1}]}}


% Method labels

\newcommand{\methodA}{{Method~A}\xspace}
\newcommand{\methodB}{{Method~B}\xspace}
\newcommand{\methodC}{{Method~C}\xspace}
\newcommand{\methodsAandB}{{Method~A and Method~B}\xspace}
\newcommand{\methodsBandC}{{Method~B and Method~C}\xspace}
\newcommand{\allmethods}{{Methods~A, B and C}\xspace}


% Basic physics commands

\newcommand{\lag}{\mathcal{L}} 
\newcommand{\TeV}{\,\mathrm{TeV}}  
\newcommand{\GeV}{\,\mathrm{GeV}}  
\newcommand{\MeV}{\,\mathrm{MeV}}  
\newcommand{\keV}{\,\mathrm{keV}}  
\newcommand{\eV}{\,\mathrm{eV}}  
\newcommand{\half}{{\frac{1}{2}}}
\newcommand{\mom}[1]{{{\vec p}_{#1}}}
\newcommand{\invfb}{\ensuremath{{\mathrm{fb}^{-1}}}}
\newcommand{\cls}{\ensuremath{{CL_s}}\xspace}
\newcommand{\clsb}{\ensuremath{{CL_{s+b}}}\xspace}
\newcommand{\clb}{\ensuremath{{CL_{b}}}\xspace}
\newcommand{\nll}{\ensuremath{{-\ln\mathcal{L}}}\xspace}

\DeclareRobustCommand{\pT}{\mymath{p_\MathUpright{T}}\xspace}
\newcommand{\pt}{\pT}
\newcommand{\bjet}{{\ensuremath{b\textrm{-jet}}}\xspace}
\newcommand{\bjets}{{\ensuremath{b\textrm{-jets}}}\xspace}

\RequirePackage{mathtools}
\newcommand{\defeq}{\vcentcolon=}


% Constants and other things

\newcommand{\numPseudoDatasets}{{19000}\xspace}


% Miscellaneous formatting things

\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\eqnref}[1]{equation~\eqref{eqn:#1}}
\newcommand{\tableref}[1]{Table~\ref{table:#1}}
\newcommand{\eqnsref}[2]{equations~\eqref{eqn:#1} and \eqref{eqn:#2}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\appendixref}[1]{Appendix~\ref{appendix:#1}}
\newcommand{\definemath}[2]{\def#1{\ifmmode#2\else$#2$\fi}}


% Stats distributions
\newcommand{\distN}[2]{\sim\mathcal{N}\left(#1,#2\right)}
\newcommand{\distGauss}[2]{\sim\text{Gauss}\left(#1,#2\right)}
\newcommand{\distPoiss}[1]{\sim\text{Poiss}\left(#1\right)}
\newcommand{\distUn}[2]{\sim\mathrm{Un}\left(#1,#2\right)}
\newcommand{\distGP}[1]{\sim\mathcal{GP}\left(#1\right)}


% Fake-rate estimation type commands


\newcommand\objtight{{\ensuremath{t}}\xspace}
\newcommand\objloose{{\ensuremath{l}}\xspace}
\newcommand\objreal{{\ensuremath{r}}\xspace}
\newcommand\objfake{{\ensuremath{f}}\xspace}
\newcommand\objall{{\ensuremath{\tilde l}}\xspace}

\newcommand\eventtight{{\ensuremath{T}}\xspace}
\newcommand\eventloose{{\ensuremath{L}}\xspace}
\newcommand\eventreal{{\ensuremath{R}}\xspace}
\newcommand\eventfake{{\ensuremath{F}}\xspace}
\newcommand\eventall{{\ensuremath{\tilde L}}\xspace}


\newcommand\effReal{{\ensuremath{\varepsilon_\objreal}}\xspace}
\newcommand\effFake{{\ensuremath{\varepsilon_\objfake}}\xspace}
\newcommand\effRealBar{{{\ensuremath{\bar\varepsilon}_\objreal}}\xspace}
\newcommand\effFakeBar{{{\ensuremath{\bar\varepsilon}_\objfake}}\xspace}

\newcommand\objcategory[1]{{\ensuremath{\omega_{#1}}}\xspace}
\newcommand\eventcategory[1]{{\ensuremath{\Omega_{#1}}}\xspace}

\newcommand\effRealObj[1]{{\ensuremath{\varepsilon_{\objcategory{#1} \objreal}}}\xspace}
\newcommand\effFakeObj[1]{{\ensuremath{\varepsilon_{\objcategory{#1} \objfake}}}\xspace}
\newcommand\effRealBarObj[1]{{{\ensuremath{\bar\varepsilon}_{\objcategory{#1} \objreal}}}\xspace}
\newcommand\effFakeBarObj[1]{{{\ensuremath{\bar\varepsilon}_{\objcategory{#1} \objfake}}}\xspace}

\newcommand\numlep{{\ensuremath{m}}\xspace}
\newcommand\numobjcategories{{\ensuremath{N_\omega}}\xspace}
\newcommand\numeventcategories{{\ensuremath{N_\Omega}}\xspace}

\newcommand\numObsInObjCategory[1]{{\ensuremath{n_{\objcategory{#1}}}}\xspace}
\newcommand\numObsInEventCategory[1]{{\ensuremath{n_{\eventcategory{#1}}}}\xspace}
\newcommand\numTight{{\ensuremath{n_\eventtight}}\xspace}
\newcommand\numLoose{{\ensuremath{n_\eventloose}}\xspace}
\newcommand\numFake{{\ensuremath{n_\eventfake}}\xspace}
\newcommand\numReal{{\ensuremath{n_\eventreal}}\xspace}
\newcommand\numTightFake{{\ensuremath{n_{\eventtight\eventfake}}}\xspace}
\newcommand\numTightReal{{\ensuremath{n_{\eventtight\eventreal}}}\xspace}
\newcommand\rateTight{{\ensuremath{\nu_\eventtight}}\xspace}
\newcommand\rateLoose{{\ensuremath{\nu_\eventloose}}\xspace}
\newcommand\rateReal{{\ensuremath{\nu_\eventreal}}\xspace}
\newcommand\rateFake{{\ensuremath{\nu_\eventfake}}\xspace}
\newcommand\rateTightFake{{\ensuremath{\nu_{\eventtight\eventfake}}}\xspace}
\newcommand\rateTightReal{{\ensuremath{\nu_{\eventtight\eventreal}}}\xspace}

\newcommand{\expectation}[1]{{\ensuremath{\mathbb{E}\left[ {#1} \right]}}}
\newcommand{\expected}[1]{{\ensuremath{\left< {#1} \right>}}}
\newcommand{\expn}[1]{{\ensuremath{\expected{n_{#1}}}}}

\newcommand{\fakephi}[3]{{\ensuremath{{\phi_\objcategory{#1}}_{#2}^{\ #3}}}\xspace}
\newcommand{\fakeinvphi}[3]{{\ensuremath{{\phi^{-1}_\objcategory{#1}}_{#2}^{\ #3}}}\xspace}
\newcommand{\fakePhi}[3]{{\ensuremath{{\Phi_{\bm{#1}}}_{\bm{#2}}^{\ \bm{#3}}}}\xspace}
\newcommand{\fakeinvPhi}[3]{{\ensuremath{{\Phi^{-1}_{\bm{#1}}}_{\bm{#2}}^{\ \bm{#3}}}}\xspace}

\newcommand\ntfhat{{\ensuremath{\hat n_{TF}}}\xspace}

\newcommand\tensTL{{\ensuremath{n_\mathcal{T}}}\xspace}
\newcommand\tensRF{{\ensuremath{n_\mathcal{R}}}\xspace}
\newcommand\tensRFHat{{\ensuremath{{\hat n}_\mathcal{R}{}}}\xspace}
\newcommand\tensTLHatFake{{\ensuremath{{{\hat n}_\mathcal{T}}^\eventfake{}}}\xspace}

\newcommand\tensRateTL{{\ensuremath{\nu_\mathcal{T}}}\xspace}
\newcommand\tensRateRF{{\ensuremath{\nu_\mathcal{R}}}\xspace}
\newcommand\tensRateMLETL{{\ensuremath{\nu_{\mathcal{T},\text{MLE}}}}\xspace}
\newcommand\tensRateMLERF{{\ensuremath{\nu_{\mathcal{R},\text{MLE}}}}\xspace}


% Theorem stuff - maybe not needed

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\newenvironment{proof}[1][Proof]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{definition}[1][Definition]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newcommand{\qed}{\nobreak \ifvmode \relax \else
      \ifdim\lastskip<1.5em \hskip-\lastskip
      \hskip1.5em plus0em minus0.5em \fi \nobreak
      \vrule height0.75em width0.5em depth0.25em\fi}

